AI-Slop to AI-Polish? Aligning Language Models through Edit-Based Writing Rewards and Test-time Computation

AI-generated text is proliferating across domains, from creative writing and journalism to marketing content and scientific articles. Models can follow user-provided instructions to generate coherent and grammatically correct outputs but in this work, we study a more fundamental question: how do we evaluate and improve the writing quality of AI-generated text? Writing quality assessment has received less attention from the community, in part because it is fundamentally subjective and requires expertise. We first introduce the Writing Quality Benchmark (WQ) by consolidating five writing-preference datasets into 4,729 writing quality judgments. Our experiments show that most of the competitive baselines, including state-of-the-art LLMs that excel at reasoning tasks, barely outperform random baselines on WQ. We then train specialized Writing Quality Reward Models (WQRM) of various sizes for writing quality assessment that demonstrate strong generalization on four out-of-distribution test sets and 74% accuracy on the WQ benchmark. To further show WQRM's practical benefits during inference, we leverage additional test-time compute to generate and rank multiple candidate revisions, allowing us to select higher-quality outputs from an initial draft. Human evaluation with 9 experienced writers confirm that WQRM-based selection produces writing samples preferred by experts 66% overall, and 72.2% when the reward gap is larger than 1 point. We release our datasets and models to encourage community engagement with writing quality assessment and development of AI writing systems better aligned with human preferences.

==> dump.tex <==
% \jw{since this is a debatable and emerging area, let's add another side of voice here to showcase the conflict, either ways lead to the need: we need a human-aligned reward model. For example, work related to AI's Self-Anthropomorphism like https://arxiv.org/pdf/2410.03870 and https://arxiv.org/pdf/2210.12429 which argue that AI doesn't need to sound like human, depends on the use cases. Other good sides mentioned in https://arxiv.org/pdf/2403.12004}

% The first paragraph is generated with one of three LLMs (from the LLama, GPT, or Claude families) and the second is an expert-edited version of the first with the aim to improve writing quality and remove idiosyncracies common in AI writing. Besides an implicit preference that can be assigned with each pair (i.e., the expert-edited paragraph has higher writing quality than the AI-generated one), experts also assigned explicit \textit{quality scores} (scale 1-10) to each of the paragraphs. 

% For training generative reward model we rely on the Llama 3 model family.
% In particular we instruction tuned Llama3.1 70B  on the P, R and PR training sets in a parameter efficient way with QLora \cite{dettmers2023qlora} and FSDP \cite{zhao2023pytorch} optimizing standard cross entropy loss. Table \ref{tab:json-examples} in Appendix show the training instructions for P and R setting. For PR we combine training instructions from both P and R and train in a multitask fashion. From 1000 training samples we discarded 154 samples for training P style reward models where the difference between the Initial and Final Writing quality z-score was less than 1.0. To account for positional bias prevalent in LLM evaluation \citep{li2023split,shi2024judging,zheng2023judging} each pairwise example is duplicated to contain its commutator along with the original (AB \& BA). This resulted in 1692 samples for training pairwise reward models. For training scalar reward models we use all 2000 samples (1000 pairs). For training PR models we combined $P_{train}$ and $R_{train}$ resulting in 3692 samples.

% \paragraph{Rationales in Input/Output} For the IR$\rightarrow$O setup during fine-tuning we augment each input (P or R style) as shown in Table \ref{tab:json-examples} with ``\textbackslash n\textbackslash n Some Thoughts : \{\{rationale\}\}''. During inference we just provide the input. We posit the model learns strong signals through fine-tuning with rationales that helps it provide improved rewards even without rationale at inference time.For the I$\rightarrow$OR setup during fine-tuning we modify the output such that model should first justify its rationale followed by its preference. This is the standard Chain-Of-Thought paradigm


% Prior work on evaluating the writing abilities of LLMs has differed in approach on several important criteria such as the evaluation task (pairwise preference vs. reward assignment), the length of response to evaluate, whether to rely on experts or crowdsourcing for annotation, or the writing domain (fiction, non-fiction historical, news, etc.). In the benchmark we leverage five datasets to maintain the diversity of perspectives represented in past work while standardizing the evaluation format into a pairwise preference to consolidate evaluation. Specifically, each of the 5,000 samples in WQ consists of two writing responses, and a binary label for which of the two is considered better in terms of writing quality. The aim of the Writing Quality benchmark is to determine which reward models are capable of assessing writing quality most generally, independent of domain, response length, or perspective.

% We first describe the salient properties that exist in prior work on writing evaluation, and then introduce each of the five datasets we selected for WQ and the property they bring to the benchmark. Table~\ref{todo} summarizes these salient properties and the composition of the benchmark.

%Too lengthy
% \subsection{Properties of Writing Quality Benchmarks}

% \paragraph{Origin of Responses.} The text responses being evaluated can be obtained in various ways: entirely manual written of a person (Human), generated in a fully-automatic way using an AI system, or through a human-in-the-loop Human-AI collaboration. Some prior work, such as LM Arena, focuses on obtaining judgments of AI vs. AI writing, whereas other work such as Art or Artifice requires a comparison of human-written text to AI-generated text for a common writing instruction. We argue that the origin of the text responses is a crucial dimension to writing quality assessment, and ensure that the benchmark includes a diverse set of combinations: AI-AI, Human-AI, Human-Human, and AI-HumanAI.

% \paragraph{Annotator Level of Expertise.} Writing assessment is a technical topic taught in specialized graduate programs (such as Masters of Fine Arts). As such, prior work has argued that writing quality evaluation should engage domain experts and work with editors or published authors. On the other hand, writing and reading are part of daily lives for many, and some work has leveraged crowdsourcing or unpaid volunteers to assess preference in writing. We include in our benchmark four datasets based on expert opinion, and one based on crowdsourcing to adequately represent both perspectives.

% \paragraph{Length of Responses.} Creative writing is challenging both in short form (e.g., writing an engaging paper title) and long-form (e.g., writing a published New Yorker story). However, increased response length is challenging in NLP for practical reasons: first, longer responses require additional time and effort from annotators, and second LLMs are known to deteriorate in abilities in long-context settings. Due to these practical considerations, prior work has predominantly focused on short-form evaluation, which we define as responses with less than 500 words. Some prior work has however focused specifically on long-form generation (1500-2500 words), which we include in the benchmark, ensuring that both long-form and short-form generation are represented in the benchmark.

% We next cover how each dataset was processed into a standardized format to produce the 5,000 final samples in the WQ benchmark.

% either through generation by an AI system, or by manual writing from a human with varied levels of experience with writing. Some prior work, such as LM Arena, has producing AI-AI comparisons, by focusing on AI-generated responses. On the other hand, others have assessed human-AI 

% We now describe the procedure we followed to build the Writing Quality benchmark. We first go over the desired properties for the benchmark, and then describe how we processed five existing datasets to produce a general benchmark for writing quality. Our selection process purposefully includes datasets that vary on important properties, ensuring that a method that achieves strong performance on the benchmark 

% There aren't enough datasets to evaluate writing quality in a pairwise fashion. The few datasets that exists predominantly compares $<$AI-AI$>$ writing pairs. By limiting focus on only AI-AI comparisons without considering human writing these datasets create a blind spot in real world applications. Additionally the judgment for pairwise preferences are collected primarily via crowd-sourcing. This introduces inconsistency and potential biases as non-expert evaluators often lack the skills to assess the nuanced aspects of writing quality. To account for this we benchmark our reward models on 5 distinct writing preference datasets. Our test datasets offer different degree of contrasts. For instance in \textbf{LAMP-test} there are not only $<AI-AI>$ pairs but also $<AI-HumanAI>$ pairs which reflects human-AI collaboration. \textbf{Synthetic Mirror AI} and \textbf{Human Mirror MFA} on the other hand test if LLMs can reward expert quality writing over its other counterpart. And finally  \textbf{Art or Artifice} stress tests our reward models on generalization over length.

% Authors of the work focused on evaluating writing quality in the domain of flash fiction writing: fictional stories that typically span 1,500-2,500 words. Evaluation data consists of 12 writing instructions based on original flash fiction stories published in the \textit{New Yorker}. Each plot is then associated with four responses: the original New Yorker story, and three LLM-generated stories (by GPT-3.5, GPT4, and Claude). For each plot, three annotators with writing expertise read all four story responses, and ranked them according to preference. The authors of work 10 aggregated the ranks into a majority vote such that for any pair of stories on a common plot, a majority preference is known. For each plot, we consider the six pairs of responses (4C2), and use the expert majority vote as the preference label. Leveraging the 12 story plots and all response combinations, we obtain a total of 144 preference samples (by duplicating each pair into an AB and BA order). Note that 25\% of samples in this dataset are Human-AI comparisons, while 75\% are AI-AI comparisons.

% The test set of the LAMP corpus focuses on short-form creative writing (200-400 word) including both fiction and non-fiction writing instructions. The test set consists of 201 samples called triplets. A triplet consists of a writing instruction and three responses: (1) an AI-written response, (2) an AI-written+AI-edited response, (3) an AI-written+AI-edited response. The triplets were ranked by three professionals with expertise in writing for preference, and authors of the work combined individual writer ranks into a single majority vote. For each writing instruction, we consider the 3 pairs of responses (3C2) and include use of the expert majority vote as the preference label. The 201 triplets yield a total of 1206 samples (by duplicating each pair into an AB  and BA order). Note that 33\% of samples in this dataset are AI-HumanAI comparisons, while 66\% are AI-AI comparisons.

% whether MFA students could mimic the style of an award-winning author. Specifically, 28 MFA students were given 20 samples written by an award-winning author (such as Haruki Murakami, Yoko Ogawa, Percival Everett, Zadie Smith, Joan Didion), their style, and a writing instruction matching an unrevealed passage from the author. The MFA students were then tasked with completing the writing instruction (typically 200-400 words) while imitating the style of the author to the best of their ability. In total, 150 samples were collected: consisting of a writing instruction, and a pair of writing responses (by the MFA student, and the original author). We include all 150 pairs in as part of the benchmark, and assign an implicit preference for the original author's response (i.e., assuming that the MFA-written imitation is worse than the original). Note that all samples in Mirror Human are Human-Human comparisons.

% Prior work on AI-detection methods has introduced the concept of ``synthetic mirrors'', a two-step approach to generating pairs of writing responses with a known implicit preference. First, a \textit{mirror prompt} is generated using an LLM by providing the LLM with an original human-written writing sample. The mirror prompt extracts both a plot summary of the writing, but also structured features such as tone, stylistic features, length, etc. In a second step, the mirror prompt can then be used to produce a \textit{syntetic mirror} (or mirror example) of the original writing sample: a response that closely resembles the semantic content and extracted features, but that is AI-generated. We follow the Synthetic Mirror response by selecting 140 original paragraphs from New Yorker-published flash fiction stories, written by award-winning authors (such as Alice Munro, Jhumpa Lahiri, and Annie Ernaux). We then generate a mirror prompt for each paragraph using Claude-3.5 Sonnet, specifically extracting a 30-word plot, the voice, person. We then devise mirror prompts the following mirror prompts: \textit{Write a \textit{n} word paragraph in the style of \textit{author} in \textit{v} voice given the content below.\textbackslash n \textit{plot}}. We generate a mirror response for each prompt using both GPT-4o and Claude-3.5 Sonnet, obtaining 280 Human-AI response pairs. For each pair, we assign an implicit preference for the author-written response. The Synthetic Mirror portion of the benchmark consists of 560 total preference pairs (as each pair is duplicated into an AB and BA order).

While the unprecedented rate of increase in AI assistance for writing cannot be stopped, it is urgent to align text generated from AI with humans. The most popular type of feedback used in post-training for aligning LLMs is binary preferences between pairs of examples sampled from one or more language models \citep{christiano2017deep}. However, this approach has a drawback. The paired outputs may differ in several ways and could be equally worse in terms of quality \citep{casper2023open,lambert2023alignment}. Asking an annotator to choose between two undesirable outputs does not improve alignment\footnote{In the current design of RLHF annotators are not allowed to not pick either}. Towards this \citet{chakrabarty2024can} argue that alignment training should consider how desirable each individual response is on its own merits, not just in comparison to other responses.

They show that identifying and editing problematic parts of responses can serve as an effective strategy for improving AI alignment. Such a strategy is deeply rooted in the cognitive process model of writing \citep{hayes1987cognitive} where during \textit{Reviewing} phase humans evaluate the written text, identifying areas for improvement, and making revisions. They release a high quality corpus called LAMP (Language model Authored, Manually Polished) consisting of 1282 $<AI-generated, Expert-Edited>$ pairs with implicit preference ($edited> original\_draft$) to improve AI writing (See Table \ref{ai_edit}). Additionally each AI-generated and Expert-Edited paragraph comes with normalized writing quality scores (scale 1-10) that avoids some of the inherent subjectivity that comes with quantifying, qualitative tasks such as writing.

Our work builds on top of this data. As a first step we train Writing Quality Reward Models (WQRM) across multiple model families that uses both pairwise and scalar rewards available in LAMP. However, when seeking to evaluate these models, we identified a critical gap. There aren't enough datasets to evaluate writing quality in a pairwise fashion. The few datasets that exists predominantly compares $<$AI-AI$>$ writing pairs. By limiting focus on only AI-AI comparisons without considering human writing these datasets create a blind spot in real world applications. To mitigate this we first introduce the \textit{Writing Quality Benchmark} (WQ) by consolidating five writing preference datasets that contrasts Human-Human, Human-AI and AI-AI pairs. Additionally, we implement a teacher-student knowledge distillation approach where we fine-tune open weight generative models (students) on LAMP with silver rationales generated from stronger LLMs (teachers) for rewarding writing quality (Section \ref{rationalereward}). This framework enhances model faithfulness and robustness against spurious cues by transferring reasoning abilities from from the more powerful teacher models to the more efficient student models. Empirical results show that these reward models trained on LAMP outperform both  proprietary closed-sourced LLMs such as GPT4o, GPT4o1 \citep{openai2024o1} and open weight models like DeepSeek-R1 \cite{guo2025deepseek} as well as competitive models on RewardBench such as Skywork-Reward. \citep{liu2024skywork}. 


Next we use the expert edit interaction traces from LAMP data (Figure \ref{}) to train a Chain-of-Thought based editing model. Here the model in a step-by-step manner identifies problematic spans in a draft, categorizes them, suggest span level edits and combines the edited spans to create a fresh edited paragraph. Recent work has leveraged additional computation at inference-time for improving the performance of large language models (LLMs) \citep{hosseini2024v,lightman2023let,wu2024inference,ji2025test,snell2024scaling}. Following this we employ \textit{best-of-N-sampling}, a popular approach for test-time compute \citep{chow2024inference,cobbe2021training,lightman2023let} to select the best edited paragraph based on our best performing reward model. An independent expert evaluation on responses generated from LLMs on 100 distinct writing instructions spanning across fiction, non-fiction and marketing show that expert judgment is correlated with our reward models \textbf{caveat}. Our results and empirical observations is a positive step towards improving alignment of LLMs with expert humans on subjective tasks such as writing that is one of the most common use-case of AI \citep{handaeconomic}.

% LM Arena is an academic effort evaluating various LLMs on instruction following capabilities. The effort is crowd-sourced, with unpaid users bringing their own instructions to the system and volunteering their time in reviewing a pair of responses from two randomly selected LLMs in exchange for the free use of these LLMs. Maintainers of LM Arena publicly released a corpus of anonymized instructions, accompanied by the two responses and the preference judgment. Analysis of the corpus by the authors revealed that creative writing makes up 20\% of the instructions in the corpus, indicating that creative writing is one of the three most common interactions by LM Arena users. From the roughly 100,000 samples released in the corpus that were tagged as creative writing related, we filter responses that are: (1) in English, (2) where the annotator assigned a non-tied preference, (3) and where each of the responses were between 100 and 2,000 words. Initial inspection of the 7,981 samples that match all criteria revealed that many of the samples did not match a strict definition of creative writing (e.g., ``todo''). To validate the quality of the samples in the dataset, we implement a secondary filtering stage using GPT-4o. We manually annotated 10 instructions that matched our definition for a creative writing sample task, and 10 that did not. We then compiled the 20 examples into a few-shot prompt and used GPT-4o to classify all instructions. This secondary filtering stage yielded, a total of 1,959 pairs. Due to LM Arena being larger in scale than other datasets in the benchmark, we do not include both order variants (AB/BA) in the dataset, but ensure that preference order is balanced within the dataset.

% In total, the five datasets included in the Writing Quality benchmark contribute 5,000 pairwise-preference samples, with diverse representations of the properties described in Section~\ref{todo}. We next describe the set of systems we included in our experiments.

% Eminent author Curtis Sittenfield has referred to ChatGPT writing as \textit{lunch from a fast-casual chain} or the \textit{literary equivalent of fat free cookie}. 

% Table \ref{reward_perf} shows the performance of different reward models across all our test sets. Its encouraging to see that both IR$\rightarrow$O and I$\rightarrow$OR models significantly outperform Llama3.1 70B models. This highlights the value of structured reasoning that can improve the alignment of LLMs towards better writing quality judgments.GPT4-o in few-shot setting outperforms the zero-shot model by a huge margin confirming prior findings on how in-context learning can lead to better alignment \citep{lin2023unlocking}.The \textbf{LMArena} test set appears to be hardest across all models, with the best performance of 56.7 being close to random. This performance might reflect the amount of noise present in crowd-sourced judgments. The \textbf{Style Mimic} test set also appears to be challenging with only ModernBert, GPT4-o fewshot and GPT4-o1 outperforming a random baseline of 50. The \textbf{Mirror Synthetic} data appears to be the easiest as finetuned reward models might pick up on the difference between AI vs Expert writing style and voice. The very low performance of GPT4o1, DeepSeek R1, and GPT4-o in the \textbf{Synthetic Mirror} test set shows some of the inherent issues in alignment. While the dataset was generated using Claude3.5Sonnet and not DeepSeekR1 recent work from \citet{chakrabarty2024can} has shown that all LLMs demonstrate similar idiosyncrasies in writing. We posit this makes it easier for LLMs to recognize and favor their own generations \citep{panickssery2024llm}. On Lamp-Test set most finetuned models get decent performance due to the data distribution being in-domain. The surprising performance comes from \textbf{Art or Artifice}. We see ModernBert models or Llama3.1 IR$\rightarrow$O achieving an accuracy of 80.5. This is impressive given our reward models were trained on much shorter paragraph-level texts and can generalize to long-form writing.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/Writing_Quality_Triplets.pdf}
%     \caption{Triplets of responses are generated by using the editing pipeline to generate 20 candidate responses and leveraging the MBERT-WQRM-PR model to select a high-scoring candidate.}
%     \label{fig:triplet_generation}
% \end{figure}


% We implement a pipeline with the same high-level architecture as they did, but with several technical differences.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/old_benchmark_results.tex <==
\begin{table*}[!ht]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|p{1.5cm}|p{1.25cm}|p{0.63cm}|p{1.6cm}|p{1.45cm}|p{1.53cm}|c|c|c|}
\hline
\textbf{Model} & \begin{tabular}[c]{@{}l@{}}\textbf{Training}\\\textbf{Mode}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Test}\\\textbf{Mode}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Lamp-Test}\\\textbf{(AI-AI \& AI} \\ \textbf{-HumanAI)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Synthetic}\\\textbf{Mirror AI} \\ \textbf{(AI-Expert)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Human}\\\textbf{Mirror MFA }\\ \textbf{(Human-}\\ \textbf{Expert)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{LM}\\\textbf{Arena}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Art or}\\\textbf{Artifice}\end{tabular} & \textbf{Avg} \\
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Llama3.1\\ (70B)\end{tabular}} & LAMP-P & P & 71.7 & 88.1 & 35.6 & 47.7 & 45.1 & 57.6 \\
\cline{2-9}
 & LAMP-R & P & 40.3 & 44.8 & 50 & 54.3 & 50 & 47.8 \\
\cline{2-9}
 & LAMP-PR & P & 71.3 & 94.8 & 40.6 & 44.3 & 52 & 60.6 \\
\hline\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Llama3.1\\ + IR$\rightarrow$O\end{tabular}} & LAMP-P \newline -exp & P & \textbf{74.9} & \textbf{100} & 43 & 52.8 & \textbf{80.5} & 70.2 \\
\cline{2-9}
 & LAMP- \newline PR-exp & P & 73.7 & 99.6 & 54.3 & 50.1 & 69.4 & 69.4 \\
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Llama3.1\\ + I$\rightarrow$OR\end{tabular}} & LAMP- \newline P-exp & P & 74.1 & 99.9 & 38.6 & 49.15 & 75.1 & 67.3 \\
\cline{2-9}
 & LAMP- \newline PR-exp & P & 71.7 & 99.1 & 42.6 & 55.2 & 76.3 & 68.9 \\
\hline\hline
\multirow{3}{*}{ModernBert} & LAMP-P & P & 71.5 & 99.02 & 64 & 49.4 & 73.6 & 71.5 \\
\cline{2-9}
 & LAMP-R & P & 70.8 & 99.64 & 65.3 & 48.2 & 77.7 & 72.3 \\
\cline{2-9}
 & LAMP-PR & P & 72.6 & 99.8 & 67.3 & 51 & \textbf{80.5} & \textbf{\color{ForestGreen}74.2} \\
\hline\hline
RWBench\newline  Skywork & Zeroshot & P & 54 & 90.1 & 33.3 & 55.2 & 68 & 60.1 \\
\hline
GPT-4o & 5-shot & P & 40.3 & 39.5 & 67.3 & 55.5 & 68.8 & 54.3 \\
\hline
o1 & Zeroshot & P & 39.8 & 25.8 & \textbf{68.6} & \textbf{56.7} & 67.3 & 51.6 \\
\hline
DeepSeekR1 & Zeroshot & P & 39.2 & 31.7 & 46.7 & \textbf{56.7} & 54.2 & 45.7 \\
\hline
GPT-4o & Zeroshot & P & 36.8 & 7.5 & 47.6 & 55.7 & 56.2 & 40.7 \\
\hline
\end{tabular}
\caption{\label{reward_perf}Performance of different reward models across all of our 5 test sets. The last column Avg represents the average performance across all datasets}
\label{tab:model_performance}
\end{table*}
